{A New Hope}: Contextual Privacy Policies for Mobile Applications and An Approach Toward Automated Generation

Privacy policies have emerged as the predominant approach to conveying privacy notices to mobile application users. In an effort to enhance both readability and user engagement, the concept of contextual privacy policies (CPPs) has been proposed by researchers. The aim of CPPs is to fragment privacy policies into concise snippets, displaying them only within the corresponding contexts within the application's graphical user interfaces (GUIs). In this paper, we first formulate CPP in mobile application scenario, and then present a novel multimodal framework, named SeePrivacy, specifically designed to automatically generate CPPs for mobile applications. This method uniquely integrates vision-based GUI understanding with privacy policy analysis, achieving 0.88 precision and 0.90 recall to detect contexts, as well as 0.98 precision and 0.96 recall in extracting corresponding policy segments. A human evaluation shows that 77% of the extracted privacy policy segments were perceived as well-aligned with the detected contexts. These findings suggest that SeePrivacy could serve as a significant tool for bolstering user interaction with, and understanding of, privacy policies. Furthermore, our solution has the potential to make privacy notices more accessible and inclusive, thus appealing to a broader demographic. A demonstration of our work can be accessed at https://cpp4app.github.io/SeePrivacy/

==> 8_ThreatsToValidity.tex <==
\section{Threats to Validity and Limitations}
\label{sec_threats}

% \noindent \textbf{Internal validity.} Threats to internal validity refer to errors in our experiments. We reuse several pre-trained classifiers to process privacy policies. We employ PP-OCR and GPT-3.5 for textual GUI element detection. We follow OpenAI’s API to access GPT-3.5. We specifically evaluate the performance of every module on the benchmark dataset. Our data and code are available at \url{https://github.com/Cpp4App/Cpp4App}. We also conduct a usability evaluation to further validate the functionality of \textsc{SeePrivacy} in practice. 

% \noindent \textbf{External validity.} Threats to external validity refer to the generalizability of our proposed method. Although our benchmark dataset covers various application categories, it is mainly composed of relatively popular mobile apps. However, we designed a set of selection rules to collect different pages in applications as completely as possible. In addition, \textsc{SeePrivacy} is based on learning-based GUI pattern understanding and privacy policy analysis, which is well-known for its generalizability. Thus, we believe there is a minimal threat to external validity.
% 


\noindent \textbf{Limitations.}
Our current usability evaluation focuses more on the functionality of \textsc{SeePrivacy}, i.e., the level of matching between contexts and retrieved policy segments, thus, all participants are relatively well-educated in technology.
Thus, the popularity of CPPs among them may be biased and under representative.
To dispel the potential bias, we plan to conduct a more balanced and large-scale user study that includes various socio-professional demographic with different levels of tech savviness in future.
In addition, the time and storage efficiency of \textsc{SeePrivacy} were evaluated theoretically and may not reflect real-world performance on mobile devices. Furthermore, the human-computer interaction (HCI) aspects and interaction design have not been fully developed or tested.
\sd{Android to iOS?}

==> 9_RelatedWork.tex <==
\section{Related Work}
\label{sec_relatedwork}

\sd{Those Vision-based GUI understanding focus more on the functions of UI widget from the perspective of developers, but our CPPs focus more on its semantic meanings, i.e., what do users perceive in terms of their privacy information?}
\noindent \textbf{Vision-based mobile GUI understanding.}
Previous researchers have been intensively studying this topic from different perspectives~\cite{white2019improving, chen2019gallery, chen2020object, xie2022psychologically}.
White et al.~\cite{white2019improving} leverage a famous object detection model called YOLOv2, to detect GUI widgets in-app screenshots for testing. 
Chen et al.~\cite{chen2019gallery} apply Faster R-CNN to obtain GUI widgets from app screenshots to construct a GUI widget gallery. 
In another work, Chen et al.~\cite{chen2020object} propose a hybrid method that combines traditional rule-based and learning-based CV techniques, achieving the start-of-the-art performance for GUI widget detection.
Xie et al.~\cite{xie2022psychologically} present a novel unsupervised image-based method for inferring perceptual groups of GUI widgets. 

\noindent \textbf{Privacy policy analysis.} \sd{Add a little bit more from S/P communities.}
Wilson et al.~\cite{wilson2016creation} build a privacy policy corpus with 23K fine-grained data practice annotations.
Kaur et al.~\cite{kaur2018comprehensive} perform a comprehensive analysis of keywords and content of over two thousand online policy documents.
Zimmeck et al.~\cite{zimmeck2019maps} introduce the
Mobile App Privacy System (MAPS) for conducting an
extensive privacy census of Android apps. The evaluation of a million Android apps reveals that existing policies are often silent on the practices performed by apps.
Amos et al.~\cite{amos2021privacy} curate a comprehensive dataset of a million privacy policies spanning over two decades, and their analyses ``paint a troubling picture'' of the privacy policy's transparency and accessibility.

%The most closet work is~\cite{windl2022automating}, called PrivacyInjector, used to automatically generate CPP for websites only. Their context detection method is intrusive and based on ad-hoc HTML analysis, which is consequently not applicable to mobile apps. In addition, their definitions of privacy-related contexts are more coarse-grained compared to this work and specific to website scenarios.

PrivacyInjector~\cite{windl2022automating} is the closest work to ours, and automatically generates CPP for websites only. However, its context detection method is intrusive and based on ad-hoc HTML analysis, thus not applicable to mobile apps. In addition, its definitions of privacy-related contexts are more coarse-grained compared to this work and specific to website scenarios.

==> Tables/50_category_level_comparison.tex <==
\begin{table}
	\begin{minipage}{0.55\linewidth}
		\caption{Category-wise overall context identification.}
		\label{tab:performance_metrics}
		\centering
\resizebox{1\linewidth}{!}{%
\begin{tabular}{lccc}
\toprule
Category  & Accuracy  & Precision & Recall  \\
\midrule
Name        & 0.98        & 0.98     & 1.00       \\
Birthday    & 1.00        & 1.00     & 1.00       \\
Address     & 0.38        & 0.41     & 0.86       \\
Phone       & 0.88        & 0.91     & 0.97       \\
Email       & 0.66        & 0.96     & 0.68       \\
Profile     & 0.70        & 0.74     & 0.93\\
Contacts    & 0.75        & 0.94     & 0.78       \\
Location    & 0.94        & 0.97     & 0.96       \\
Photos      & 0.86        & 0.98     & 0.88       \\
Voices  & 0.91       & 0.91     & 1.00       \\
Financial info   & 0.81        & 0.93     & 0.87       \\
Social media& 0.80        & 0.89     & 0.89       \\
\midrule
\textbf{Average} & 0.81 & 0.88 & 0.90 \\
\bottomrule
\end{tabular}
}%
\end{minipage}
	\hfill
	\raisebox{-0.035\totalheight}{%
	\begin{minipage}{0.4\linewidth}
		\centering
		\includegraphics[width=0.92\linewidth]{Figures/17-2.png}
		\captionof{figure}{The screenshot 17-2 after CDM.}
		\label{fig_context_cover_rate}
	\end{minipage}
	}%
\end{table}

==> Tables/category_level_comparison.tex <==
\begin{table}
	\begin{minipage}{0.55\linewidth}
		\caption{Category-wise overall context identification.}
		\label{tab:performance_metrics}
		\centering
\resizebox{1\linewidth}{!}{%
\begin{tabular}{lccc}
\toprule
Category  & Accuracy  & Precision & Recall  \\
\midrule
Name        & 0.92        & 0.92     & 1.00       \\
Birthday    & 1.00        & 1.00     & 1.00       \\
Address     & 0.38        & 0.43     & 0.79       \\
Phone       & 0.85        & 0.91     & 0.94       \\
Email       & 0.67        & 0.90     & 0.72       \\
Profile     & 0.62        & 0.64     & 0.95\\
Contacts    & 0.87        & 0.98     & 0.88       \\
Location    & 0.84        & 0.95     & 0.87       \\
Photos      & 0.78        & 0.95     & 0.81       \\
Voices  & 0.89       & 1.00     & 0.89       \\
Financial info   & 0.74        & 0.93     & 0.78       \\
Social media& 0.60        & 0.75     & 0.86       \\
\midrule
\textbf{Average} & 0.76 & 0.86 & 0.87 \\
\bottomrule
\end{tabular}
}%
\end{minipage}
	\hfill
	\raisebox{-0.035\totalheight}{%
	\begin{minipage}{0.4\linewidth}
		\centering
		\includegraphics[width=0.97\linewidth]{Figures/17-2.png}
		\captionof{figure}{The screenshot 17-2 after CDM.}
		\label{fig_context_cover_rate}
	\end{minipage}
	}%
\end{table}

% \begin{table}[ht]
% \begin{minipage}[b]{0.4\linewidth}
% \centering
% \resizebox{.95\textwidth}{!}{%
% \begin{tabular}{lccc}
% \toprule
% Category  & Accuracy  & Precision & Recall  \\
% \midrule
% Name        & 0.97        & 1.00     & 0.97       \\
% Birthday    & 1.00        & 1.00     & 1.00       \\
% Address     & 0.50        & 1.00     & 0.50       \\
% Phone       & 0.91        & 0.94     & 0.97       \\
% Email       & 0.88        & 0.88     & 1.00       \\
% Profile     & 0.66 & 0.67 & 0.98\\
% Contacts    & 0.89        & 1.00     & 0.89       \\
% Location    & 0.92        & 1.00     & 0.92       \\
% Photos      & 0.75        & 0.97     & 0.76       \\
% Voices  & 0.88       & 1.00     & 0.88       \\
% Financial info   & 0.75        & 0.92     & 0.80       \\
% Social media& 0.75        & 0.75     & 1.00       \\
% \midrule
% \textbf{Average} & 0.83 & 0.92 & 0.88 \\
% \bottomrule
% \end{tabular}
% }%
% \caption{The performance for privacy-related context identification.}
% \label{tab:performance_metrics}
% \end{minipage}
% \end{table}

% \begin{figure}[ht]
% \begin{minipage}[b]{0.35\linewidth}
% \centering
% \includegraphics[width=1.0\linewidth]{Figures/17-2.png}
% \caption{2-D scatterplot of the Student Database}
% \label{ }
% \end{minipage}
% \end{figure}


% \begin{table}[h]
% \centering
% \begin{tabular}{lccc}
% \toprule
% Category  & Accuracy  & Precision & Recall  \\
% \midrule
% Name        & 0.97        & 1.00     & 0.97       \\
% Birthday    & 1.00        & 1.00     & 1.00       \\
% Address     & 0.50        & 1.00     & 0.50       \\
% Phone       & 0.91        & 0.94     & 0.97       \\
% Email       & 0.88        & 0.88     & 1.00       \\
% Profile     & 0.66 & 0.67 & 0.98\\
% Contacts    & 0.89        & 1.00     & 0.89       \\
% Location    & 0.92        & 1.00     & 0.92       \\
% Photos      & 0.75        & 0.97     & 0.76       \\
% Voices  & 0.88       & 1.00     & 0.88       \\
% Financial info   & 0.75        & 0.92     & 0.80       \\
% Social media& 0.75        & 0.75     & 1.00       \\
% \midrule
% \textbf{Average} & 0.83 & 0.92 & 0.88 \\
% \bottomrule

% \end{tabular}
% \caption{The performance for privacy-related context identification.}
% \label{tab:performance_metrics}
% \end{table}


%The top table is icon+text, the bottom table is count by screen.
% \toprule
% Category on screenshot  & Accuracy  & Precision & Recall  \\
% \midrule
% Name        & 0.966        & 0.792     & 0.864       \\
% Birthday    & 0.983        & 1.     & 0.636       \\
% Address     & 0.966        & 1.     & 0.111       \\
% Phone       & 0.939        & 0.639     & 0.958       \\
% Email       & 0.922        & 0.667     & 0.971       \\
% Contacts    & 0.925        & 0.788     & 0.703       \\
% Location    & 0.925        & 0.763     & 0.763       \\
% Photos      & 0.850        & 0.629     & 0.815       \\
% Voices  & 0.978        & 0.6     & 0.857       \\
% Financial info   & 0.966        & 0.667     & 0.769       \\
% Social media& 0.761        & 0.127     & 1.       \\
% Profile & 0.719 & 0.446 & 0.789\\
% \bottomrule

==> Tables/evalutation_total.tex <==
\begin{table*}[!t]
\caption{Performance of SeePrivacy's modules. CDM stands for Context Detection Module.}
\label{tab_evaluation_total}
\subcaptionbox{CDM - Textual GUI components}{
\resizebox{0.2655\textwidth}{!}{%
    \begin{tabular}{lccc}
        \toprule
        \textbf{Category} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} \\
        \midrule
        Name & 0.92 & 0.92 & 1.00 \\
        Birthday  & 1.00 & 1.00 & 1.00 \\
        Address  & 0.38 & 0.43 & 0.79 \\
        Phone  & 0.90 & 0.96 & 0.93 \\
        Email  & 0.67 & 0.97 & 0.68 \\
        Profile  & 0.45 & 0.47 & 0.94 \\
        Contacts  & 0.95 & 0.98 & 0.98 \\
        Location  & 0.89 & 0.95 & 0.94 \\
        Photos  & 0.78 & 0.97 & 0.80 \\
        Voices  & 1.00 & 1.00 & 1.00 \\
        Financial info  & 0.82 & 0.93 & 0.88 \\
        Social media  & 0.60 & 0.75 & 0.75 \\
        \midrule
        \textbf{Average} & 0.78 & 0.86 & 0.89 \\
        \bottomrule
    \end{tabular}
}%
}
\hfill
\subcaptionbox{CDM - Iconic GUI components}{
\resizebox{0.328\textwidth}{!}{%
\begin{tabular}{llrrr}
\toprule
\textbf{RICO-icon Class} & \textbf{Category} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} \\
\midrule
Call  & Phone & 0.70 & 1.00 & 0.70 \\
Email  & Email & 0.74 & 0.68 & 0.81 \\
Avatar  & Profile & 0.85 & 0.82 & 0.89 \\
Follow & Contacts & 0.90 & 0.82 & 1.00 \\
Group  & Contacts &  0.67 & 0.73 & 0.62   \\
Location  & Location & 0.89 & 0.86 & 0.92 \\
Location crosshair & Location & 0.72 & 0.63 & 0.83 \\
Photo & Photos & 0.87 & 0.89 & 0.85 \\
Wallpaper  & Photos & 0.87 & 0.82  & 0.93 \\
Videocam  & Photos &  0.91 & 0.83 & 1.00 \\
Microphone  & Voices & 0.96 & 0.93  & 1.00   \\
Cart &  Financial Info & 0.81 & 0.75   &   0.88   \\
Facebook  & Social media & 0.83 & 0.75 & 0.92  \\
Twitter  & Social media & 0.90  & 0.95 & 0.86 \\
\midrule
\textbf{Average} & &  0.82 & 0.83 & 0.85  \\
\bottomrule
\end{tabular}
}%
}
\hfill
\subcaptionbox{Segments Extraction Module}{
    \resizebox{0.3465\textwidth}{!}{%
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Category}    & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{Success Rate}\\
    \midrule
    Name        & 0.98 & 0.97 & 1.00 & 0.92 \\
    Birthday    & 0.94 & 1.00 & 0.94 & 0.62 \\
    Address     & 0.48 & 0.82 & 0.50 & 0.78 \\
    Phone       & 1.00 & 1.00 & 1.00 & 0.97 \\
    Email       & 1.00 & 1.00 & 1.00 & 0.98 \\
    Profile     & 0.96 & 0.96 & 1.00 & 0.97 \\
    Contacts    & 1.00 & 1.00 & 1.00 & 1.00 \\
    Location    & 0.92 & 0.94 & 0.98 & 0.91 \\
    Photos      & 0.84 & 0.83 & 1.00 & 1.00 \\
    Voices      & 0.85 & 0.33 & 1.00 & 1.00 \\
    Financial info   & 1.00 & 1.00 & 1.00 & 0.96 \\
    Social media& 1.00 & 1.00 & 1.00 & 1.00 \\
    \midrule
    \textbf{Average} & 0.92 & 0.94 & 0.98 & 0.96  \\
    % \textbf{Average of all data types} & 0.91 & 0.90 & 0.95 & 0.99  \\
    \bottomrule
    \end{tabular}
    }%
}
\end{table*}
% check ret in gt
    % \begin{tabular}{lcccc}
    % \toprule
    % \textbf{Category}    & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{Success Rate}\\
    % \midrule
    % Name        & 0.98 & 0.97 & 1.00 & 0.92 \\
    % Birthday    & 0.94 & 1.00 & 0.94 & 1.00 \\
    % Address     & 0.48 & 0.82 & 0.50 & 1.00 \\
    % Phone       & 1.00 & 1.00 & 1.00 & 0.97 \\
    % Email       & 1.00 & 1.00 & 1.00 & 1.00 \\
    % Profile     & 0.96 & 0.96 & 1.00 & 0.97 \\
    % Contacts    & 1.00 & 1.00 & 1.00 & 1.00 \\
    % Location    & 0.92 & 0.94 & 0.98 & 1.00 \\
    % Photos      & 0.84 & 0.83 & 1.00 & 1.00 \\
    % Voices      & 0.85 & 0.33 & 1.00 & 1.00 \\
    % Financial info   & 1.00 & 1.00 & 1.00 & 1.00 \\
    % Social media& 1.00 & 1.00 & 1.00 & 1.00 \\
    % \midrule
    % \textbf{Average} & 0.92 & 0.94 & 0.98 & 0.99  \\
    % % \textbf{Average of all data types} & 0.91 & 0.90 & 0.95 & 0.99  \\
    % \bottomrule
    % \end{tabular}




% Success rate in the table below: spliting gt into phrase and calculate lcs with whole segment.
% \hfill
% \subcaptionbox{Segments Extraction Module}{
%     \resizebox{0.3465\textwidth}{!}{%
%     \begin{tabular}{lcccc}
%     \toprule
%     \textbf{Category}    & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{Success Rate}\\
%     \midrule
%     Name        & 0.98 & 0.97 & 1.00 & 0.92 \\
%     Birthday    & 0.94 & 1.00 & 0.94 & 0.62 \\
%     Address     & 0.48 & 0.82 & 0.50 & 0.78 \\
%     Phone       & 1.00 & 1.00 & 1.00 & 0.97 \\
%     Email       & 1.00 & 1.00 & 1.00 & 0.98 \\
%     Profile     & 0.96 & 0.96 & 1.00 & 0.97 \\
%     Contacts    & 1.00 & 1.00 & 1.00 & 1.00 \\
%     Location    & 0.92 & 0.94 & 0.98 & 0.91 \\
%     Photos      & 0.84 & 0.83 & 1.00 & 1.00 \\
%     Voices      & 0.85 & 0.33 & 1.00 & 1.00 \\
%     Financial info   & 1.00 & 1.00 & 1.00 & 0.96 \\
%     Social media& 1.00 & 1.00 & 1.00 & 1.00 \\
%     \midrule
%     \textbf{Average} & 0.92 & 0.94 & 0.98 & 0.96  \\
%     % \textbf{Average of all data types} & 0.91 & 0.90 & 0.95 & 0.93  \\
%     \bottomrule
%     \end{tabular}
%     }%
% }

==> Tables/interested_class.tex <==
\begin{table}[h]
\centering
\begin{tabular}{llrrr}
\toprule
\textbf{RICO-icon Class} & \textbf{Data type} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} \\
\midrule
Call  & Phone & 0.70 & 1.00 & 0.70 \\
Email  & Email & 0.74 & 0.68 & 0.81 \\
Avatar  & Profile & 0.85 & 0.82 & 0.89 \\
Follow & Contacts & 0.90 & 0.82 & 1.00 \\
Group  & Contacts &  0.67 & 0.73 & 0.62   \\
Location  & Location & 0.89 & 0.86 & 0.92 \\
Location crosshair & Location & 0.72 & 0.63 & 0.83 \\
Photo & Photos & 0.87 & 0.89 & 0.85 \\
Wallpaper  & Photos & 0.87 & 0.82  & 0.93 \\
Videocam  & Photos &  0.91 & 0.83 & 1.00 \\
Microphone  & Voices & 0.96 & 0.93  & 1.00   \\
Cart &  Financial Info & 0.81 & 0.75   &   0.88   \\
Facebook  & Social media & 0.83 & 0.75 & 0.92  \\
Twitter  & Social media & 0.90  & 0.95 & 0.86 \\
\midrule
\textbf{Average} & &  0.82 & 0.83 & 0.85  \\
\bottomrule
\end{tabular}
\caption{Performance of ours network on context-related RICO-icon classes.}
\label{tab_classification_perclass}
\end{table}

% Old model
% Call  & Phone & 0.70 & 1.00 & 0.70 \\
% Email  & Email & 0.49 & 0.55 & 0.81 \\
% Avatar  & Profile & 0.70 & 0.88 & 0.77 \\
% Follow & Contacts & 0.50 & 0.56 & 0.83 \\
% Group  & Contacts & 0.58 & 0.88 & 0.64 \\
% Location  & Location & 0.59 & 0.91 & 0.63 \\
% Location crosshair & Location & 0.77 & 0.89 & 0.86 \\
% Photo & Photos & 0.73 & 0.83 & 0.86 \\
% Wallpaper  & Photos & 0.61 & 0.70 & 0.83 \\
% Videocam  & Photos & 0.71 & 0.83 & 0.83 \\
% Microphone  & Voices & 0.93 & 0.96 & 0.96 \\
% Facebook  & Social media & 0.68 & 0.85 & 0.77 \\
% Twitter  & Social media & 0.95 & 0.95 & 1.00 \\
% \midrule
% \textbf{Average} & & 0.69 & 0.81 & 0.81    \\
% Location crosshair & Location & 0.774 & 0.889 & 0.857 \\
% Photo & Photos & 0.731 & 0.826 & 0.864 \\
% Facebook  & Social media & 0.680 & 0.850 & 0.773 \\
% Microphone  & Voices & 0.931 & 0.964 & 0.964 \\
% Email  & Email & 0.486 & 0.548 & 0.810 \\
% Twitter  & Social media & 0.952 & 0.952 & 1.000 \\
% Location  & Location & 0.594 & 0.905 & 0.633 \\
% Call  & Phone & 0.696 & 1.000 & 0.696 \\
% Wallpaper  & Photos & 0.609 & 0.700 & 0.824 \\
% Follow & Contacts & 0.500 & 0.560 & 0.824 \\
% Group  & Contacts & 0.583 & 0.875 & 0.636 \\
% Avatar  & Profile & 0.698 & 0.88 & 0.772 \\
% Videocam  & Photos & 0.714 & 0.833 & 0.833 \\
% Play  & Example 14 & 0.800 & 0.897 & 0.881 \\


==> Tables/keywords_icons_match.tex <==
\begin{figure*}[htbp]
\centering
\begin{spacing}{} 
\setlength\tabcolsep{1pt} 
\begin{tabular}{ccc}
             Privacy-related information & Icon   \\
\hline
Camera & \begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/camera1.png}}\end{minipage} &     
		\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/camera2.png}}
	\end{minipage}               \\ \\
Camera &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/camera3.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/camera4.png}}
	\end{minipage}              \\ \\
 Email &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/email1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/email2.png}}
	\end{minipage}              \\ \\
 Location &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/location1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/location2.png}}
	\end{minipage}              \\ \\
Contacts &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/contacts1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/contacts2.png}}
	\end{minipage}              \\ \\
 Contacts &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/contacts3.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/contacts4.png}}
	\end{minipage}              \\ \\
 Financial information &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/financial1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/finantial2.png}}
	\end{minipage}              \\ \\
 Microphone &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/microphone1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/microphone2.png}}
	\end{minipage}              \\ \\
 Personal identifier &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/profile1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/profile2.png}}
	\end{minipage}              \\ \\
 Phone &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/phone1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/phone2.png}}
	\end{minipage}              \\ \\
 Social Media &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/social1.png}}
	\end{minipage} &      
	\begin{minipage}[b]{0.15\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{Figures/social2.png}}
	\end{minipage}              \\ \\

\end{tabular}
\end{spacing}

\vspace{2em}
\label{tab_match}
\caption{Matching of CPP-related privacy keywords and icons.}
\end{figure*}

==> Tables/keywords_summary.tex <==
\begin{table*}[!t]
  \caption{Important data types exist in the literature.}
  \vspace{-5pt}
  \label{tab_survey}
  \centering
  \resizebox{.9\textwidth}{!}{%
  \begin{tabular}{l|cccccc|cccccc}
    \hline
    \rowcolor{lightgray!15}
    &                                                                                        \multicolumn{6}{c|}{Basic Personal Identifiable Information}                                                                       & \multicolumn{6}{c}{Other Personal Information}                                                                                     \\ 
    \hline
    \rowcolor{lightgray!85}
    &Name & Birthday & Address & Phone & Email &Profile
    & Contacts & Location & Photos & Voices & Financial Info 
    & Social Media \\
    \hline
    
    \rowcolor{lightgray!50}
    \textbf{Administration}
    & & & & & & & & & & & &\\
    \rowcolor{lightgray!15}
    GDPR~\cite{GDPR} 
    & \CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE
    & \Circle &\Circle &\Circle &\Circle &\Circle &\Circle 
    \\
    \rowcolor{lightgray!15}
    CCPA~\cite{CCPA} 
    & \CIRCLE &\Circle &\Circle &\Circle &\CIRCLE &\CIRCLE
    & \Circle &\CIRCLE &\Circle &\Circle &\CIRCLE &\Circle 
     \\
    \rowcolor{lightgray!15}
    CalOPPA~\cite{CalOPPA} 
    & \CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE &\Circle
    & \Circle &\CIRCLE &\Circle &\Circle &\CIRCLE&\CIRCLE 
    \\
    \rowcolor{lightgray!15}
    COPPA~\cite{COPPA} 
    & \CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE
    & \Circle &\CIRCLE &\CIRCLE &\CIRCLE &\Circle&\Circle 
    \\
    
    \rowcolor{lightgray!15}
    APP~\cite{APP} 
    &\CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE &\CIRCLE
    &\Circle &\CIRCLE &\CIRCLE &\Circle &\CIRCLE &\Circle
    \\
    
    \rowcolor{lightgray!50}
    \textbf{Industry}
    & & & & & &  & & & & & & \\
    \rowcolor{lightgray!15}
    Google~\cite{googledatasafety} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    \\
    % Google contains the MAC address
    \rowcolor{lightgray!15}
    Apple~\cite{appleprivacy} 
    & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    \\
    \rowcolor{lightgray!15}
    Huawei~\cite{Huaweiprivacy} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE 
    \\
    \rowcolor{lightgray!15}
    Amazon~\cite{Amazonprivacy} 
    & \Circle & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    \\
    
    \rowcolor{lightgray!50}
    \textbf{Academia} &&&&&& &&&&&&\\
    \rowcolor{lightgray!15}
    Yu et al.~\cite{yu2015autoppg} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
    \\
    \rowcolor{lightgray!15}
    Wilson et al.~\cite{wilson2016creation} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \Circle & \Circle & \CIRCLE & \CIRCLE
    \\
    \rowcolor{lightgray!15}
    Harkous et al.~\cite{harkous2018polisis} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \Circle & \Circle & \CIRCLE & \CIRCLE
    \\
    \rowcolor{lightgray!15}
    Kaur et al.~\cite{kaur2018comprehensive} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE  & \Circle
    \\
    \rowcolor{lightgray!15}
    Yu et al.~\cite{yu2018enhancing}
    & \Circle & \Circle & \Circle & \Circle & \Circle & \CIRCLE
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
    \\
    \rowcolor{lightgray!15}
    Zimmeck et al.~\cite{zimmeck2019maps} 
    & \Circle & \Circle & \Circle & \CIRCLE & \CIRCLE & \CIRCLE
    & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE
    \\
    \rowcolor{lightgray!15}
    Zhang et al.~\cite{zhang2020does} 
    & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle
    & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle
    \\
    \rowcolor{lightgray!15}
    Sun and Xue~\cite{sun2020quality} 
    & \CIRCLE & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle
    & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle
    \\
   
    \rowcolor{lightgray!15}
    Li et al.~\cite{li2021developers} 
    & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
    \\
    % \rowcolor{lightgray!15}
    % Only focus on analytics libraries rather than apps
    % Caputo et al.~\cite{caputo2021you} 
    % & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE 
    % & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
    % & \CIRCLE & \Circle\\

    \rowcolor{lightgray!15}
    Zimmeck et al.~\cite{zimmeck2021privacyflash} 
    & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle
    & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \CIRCLE
    \\
     
    \rowcolor{lightgray!15}
    Xie et al.~\cite{xie2022scrutinizing} 
    & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
    & \CIRCLE & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle
    \\
  \hline
\end{tabular}
}%
\vspace{-14pt}
\end{table*}


% \begin{table*}[!t]
%   \caption{Important data types existence in literature.}
  
%   \label{tab_survey}
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l|ccccc|cccccc|cc}
%     \hline
%     \rowcolor{lightgray!15}
%     &                                                                                        \multicolumn{5}{c|}{Basic Personal Identifiable Information}                                                                       & \multicolumn{6}{c|}{Other Personal Information}                                                                                     & \multicolumn{2}{l}{Online Identifiers} \\ 
%     \hline
%     \rowcolor{lightgray!85}
%     &Name & Birthday & Address & Phone & Email 
%     & Contacts & Location & Photos & Voices & Financial Info 
%     & Social Media &IP & Cookies \\
%     \hline
    
%     \rowcolor{lightgray!50}
%     \textbf{Administration}
%     & & & & & & & & & & & & &\\
%     \rowcolor{lightgray!15}
%     GDPR~\cite{GDPR} 
%     & \CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE 
%     & \Circle &\Circle &\Circle &\Circle &\Circle &\Circle 
%     & \CIRCLE &\CIRCLE\\
%     \rowcolor{lightgray!15}
%     CCPA~\cite{CCPA} 
%     & \CIRCLE &\Circle &\Circle &\Circle &\CIRCLE 
%     & \Circle &\CIRCLE &\Circle &\Circle &\CIRCLE &\Circle 
%     & \Circle &\Circle \\
%     \rowcolor{lightgray!15}
%     CalOPPA~\cite{CalOPPA} 
%     & \CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE 
%     & \Circle &\Circle &\Circle &\Circle &\Circle&\Circle 
%     & \CIRCLE &\CIRCLE\\
%     \rowcolor{lightgray!15}
%     COPPA~\cite{COPPA} 
%     & \CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE 
%     & \Circle &\CIRCLE &\CIRCLE &\CIRCLE &\Circle&\Circle 
%     & \CIRCLE &\CIRCLE\\
    
%     \rowcolor{lightgray!15}
%     APP~\cite{APP} 
%     &\CIRCLE &\Circle &\CIRCLE &\CIRCLE &\CIRCLE 
%     &\Circle &\CIRCLE &\CIRCLE &\Circle &\CIRCLE &\Circle
%     &\CIRCLE &\Circle\\
    
%     \rowcolor{lightgray!50}
%     \textbf{Industry}
%     & & & & & & & & & & & & &\\
%     \rowcolor{lightgray!15}
%     Google~\cite{googledatasafety} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
%     & \Circle & \Circle\\
%     % Google contains the MAC address
%     \rowcolor{lightgray!15}
%     Apple~\cite{appleprivacy} 
%     & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
%     & \CIRCLE & \Circle\\
%     \rowcolor{lightgray!15}
%     Huawei~\cite{Huaweiprivacy} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE
%     & \CIRCLE & \Circle\\
%     Amazon~\cite{} 
%     & \\
    
%     \rowcolor{lightgray!50}
%     \textbf{Academia} &&&&& &&&&&& &&\\
%     \rowcolor{lightgray!15}
%     Yu et al.~\cite{yu2015autoppg} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
%     & \CIRCLE & \CIRCLE\\
%     \rowcolor{lightgray!15}
%     Wilson et al.~\cite{wilson2016creation} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \CIRCLE & \CIRCLE & \Circle & \Circle & \CIRCLE  & \CIRCLE
%     & \CIRCLE & \CIRCLE\\
%     \rowcolor{lightgray!15}
%     Harkous et al.~\cite{harkous2018polisis} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \CIRCLE & \CIRCLE & \Circle & \Circle & \CIRCLE  & \CIRCLE
%     & \CIRCLE & \CIRCLE\\
%     \rowcolor{lightgray!15}
%     Kaur et al.~\cite{kaur2018comprehensive} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE  & \Circle
%     & \CIRCLE & \Circle\\
%     \rowcolor{lightgray!15}
%     Yu et al.~\cite{yu2018enhancing}
%     & \Circle & \Circle & \Circle & \Circle & \Circle
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
%     & \Circle & \Circle\\
%     \rowcolor{lightgray!15}
%     Zimmeck et al.~\cite{zimmeck2019maps} 
%     & \Circle & \Circle & \Circle & \CIRCLE & \CIRCLE 
%     & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle
%     & \Circle & \CIRCLE\\
%     \rowcolor{lightgray!15}
%     Zhang et al.~\cite{zhang2020does} 
%     & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle
%     & \CIRCLE & \CIRCLE\\
%     \rowcolor{lightgray!15}
%     Sun and Xue~\cite{sun2020quality} 
%     & \CIRCLE & \Circle & \Circle & \CIRCLE & \CIRCLE 
%     & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle
%     & \CIRCLE & \CIRCLE\\
   
%     \rowcolor{lightgray!15}
%     Li et al.~\cite{li2021developers} 
%     & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
%     & \CIRCLE & \Circle\\
%     % \rowcolor{lightgray!15}
%     % Only focus on analytics libraries rather than apps
%     % Caputo et al.~\cite{caputo2021you} 
%     % & \CIRCLE & \Circle & \CIRCLE & \CIRCLE & \CIRCLE 
%     % & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \Circle
%     % & \CIRCLE & \Circle\\

%     \rowcolor{lightgray!15}
%     Zimmeck et al.~\cite{zimmeck2021privacyflash} 
%     & \Circle & \Circle & \Circle & \Circle & \Circle 
%     & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & \Circle & \CIRCLE
%     & \Circle & \Circle\\
     
%     \rowcolor{lightgray!15}
%     Xie et al.~\cite{xie2022scrutinizing} 
%     & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE 
%     & \CIRCLE & \CIRCLE & \Circle & \Circle & \CIRCLE  & \Circle
%     & \CIRCLE & \CIRCLE\\
%   \hline
% \end{tabular}
% }%
% \end{table*}

==> Tables/ocr_llm_evaluation.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{lccc}
        \hline
        \textbf{Category} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} \\
        \hline
        Name & 0.62 & 0.63 & 0.98 \\
        Birthday  & 1.00 & 1.00 & 1.00 \\
        Address  & 0.47 & 0.50 & 0.89 \\
        Phone  & 0.77 & 0.82 & 0.93 \\
        Email  & 0.67 & 0.97 & 0.68 \\
        Profile  & 0.51 & 0.58 & 0.82 \\
        Contacts  & 0.95 & 0.98 & 0.98 \\
        Location  & 0.87 & 0.89 & 0.97 \\
        Photos  & 0.59 & 0.98 & 0.60 \\
        Voices  & -- & -- & -- \\
        Financial info  & 0.78 & 0.93 & 0.82 \\
        Social media  & 0.50 & 0.58 & 0.78 \\
        \hline
        \textbf{Average} & 0.70 & 0.81 & 0.86 \\
        \hline
    \end{tabular}
    \vspace{-5pt}
    \caption{CDM - Textual GUI components}
    \label{tab:ocr_llm_apr}
\end{table}

==> Tables/segment_success_rate.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|ccc|c}
\toprule
\textbf{Category}    & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{Success Rate}\\
\midrule
Name        & 0.98 & 0.97 & 1.00 & 0.92 \\
Birthday    & 0.94 & 1.00 & 0.94 & 1.00 \\
Address     & 0.48 & 0.82 & 0.50 & 1.00 \\
Phone       & 1.00 & 1.00 & 1.00 & 0.97 \\
Email       & 1.00 & 1.00 & 1.00 & 1.00 \\
Profile     & 0.96 & 0.96 & 1.00 & 0.97 \\
Contacts    & 1.00 & 1.00 & 1.00 & 1.00 \\
Location    & 0.92 & 0.94 & 0.98 & 1.00 \\
Photos      & 0.84 & 0.83 & 1.00 & 1.00 \\
Voices      & 0.85 & 0.33 & 1.00 & 1.00 \\
Financial info   & 1.00 & 1.00 & 1.00 & 1.00 \\
Social media& 1.00 & 1.00 & 1.00 & 1.00 \\
\midrule
\textbf{Average} & 0.92 & 0.94 & 0.98 & 0.99  \\
\bottomrule
\end{tabular}
\caption{Performance of the Segments Extraction Module on the benchmark dataset.}
\label{tab_segment_extraction}
\end{table}

==> Tables/total_detection_results.tex <==
\begin{table}[h]
\centering
\caption{Performance of Overall Context Identification.}
\label{tab_success_rates}
\begin{tabular}{lc}
\toprule
\textbf{GUI category} & \textbf{average Context Coverage per screenshot} \\
\midrule
Text     & 87.53\% \\
Icon     & 40.60\% \\
\midrule
\textbf{Overall}  & 83.59\% \\
\bottomrule
\end{tabular}
\end{table}




% \begin{table}[h!]
% \centering
% \begin{tabular}{@{}lcc|cc@{}}
% \toprule
%                            & \multicolumn{2}{c}{\textbf{Without Classification}} & \multicolumn{2}{c}{\textbf{With Classification}} \\ \cmidrule(lr){2-3} \cmidrule(l){4-5} 
% \textbf{}                 & \textbf{Precision}          & \textbf{Recall}          & \textbf{Precision}         & \textbf{Recall}          \\ \midrule
% \textbf{Overall}          &              0.1101               &           0.8225               &       0.4977                     &           0.6605               \\
% \textbf{Text}             &              0.1544               &            0.8646              &           0.1933                 &                0.9109          \\
% \textbf{Icon}             &             0.0913                &            0.7211              &           0.2595                 &              0.3579            \\ \bottomrule
% \end{tabular}
% \caption{Precision and recall for detection}
% \label{tab:detection_results}
% \end{table}

==> Tables/user_study_results.tex <==
\begin{table}[!t]
\centering
\caption{Statistic results of our user study. SD stands for standard deviations.}
\label{tab_user_study_results}
\resizebox{.8\linewidth}{!}{%
\begin{tabular}{llrcc}
\toprule
\textbf{No.} & \textbf{Topic} & \textbf{Mean}  & \textbf{Median}  & \textbf{SD}\\
\midrule
$\textit{Q}_1$  & Privacy concerns (-)    & 4.13 & 4 &  1.09\\
$\textit{Q}_4$  & CPP usefulness (+)  & 4.53 & 5 & 0.62 \\
\midrule
\midrule
$\textit{Q}_3$  & PP Reading frequency    &2.00 & 2 & 1.03 \\
$\textit{Q}_5$  & CPP Reading frequency    & 4.07 & 4 & 0.85 \\
\midrule
\multicolumn{2}{l}{\textbf{Improvement}} & \textbf{+2.07} & \textbf{+2} & / \\
\bottomrule
\end{tabular}
}%
\end{table}
